A Generic Inverted Index Framework for Similarity Search on the GPU - Technical Report

We propose a novel generic inverted index framework on the GPU (called GENIE), aiming to reduce the programming complexity of the GPU for parallel similarity search of different data types. Not every data type and similarity measure are supported by GENIE, but many popular ones are. We present the system design of GENIE, and demonstrate similarity search with GENIE on several data types along with a theoretical analysis of search results. A new concept of locality sensitive hashing (LSH) named $\tau$-ANN search, and a novel data structure c-PQ on the GPU are also proposed for achieving this purpose. Extensive experiments on different real-life datasets demonstrate the efficiency and effectiveness of our framework. The implemented system has been released as open source.

==> hyphenex/ushyphex.tex <==
% Hyphenation exceptions for US English,
% based on hyphenation exception log articles in TUGboat.
%
% Copyright 2008 TeX Users Group.
% You may freely use, modify and/or distribute this file.
%
% This is an automatically generated file.  Do not edit!
%
% Please contact the TUGboat editorial staff <tugboat@tug.org>
% for corrections and omissions.

\hyphenation{
  acad-e-my
  acad-e-mies
  ac-cu-sa-tive
  acro-nym
  acro-nyms
  acryl-amide
  acryl-amides
  acryl-alde-hyde
  acu-punc-ture
  acu-punc-tur-ist
  add-a-ble
  add-i-ble
  adren-a-line
  aero-space
  af-ter-thought
  af-ter-thoughts
  agron-o-mist
  agron-o-mists
  al-ge-bra-i-cal-ly
  am-phet-a-mine
  am-phet-a-mines
  anach-ro-nism
  anach-ro-nis-tic
  an-a-lyse
  an-a-lysed
  analy-ses
  analy-sis
  an-eu-rysm
  an-eu-rysms
  an-eu-rys-mal
  an-iso-trop-ic
  an-iso-trop-i-cal-ly
  an-isot-ro-pism
  an-isot-ropy
  an-ni-ver-sary
  an-ni-ver-saries
  anom-a-ly
  anom-a-lies
  anti-deriv-a-tive
  anti-deriv-a-tives
  anti-holo-mor-phic
  an-tin-o-my
  an-tin-o-mies
  anti-nu-clear
  anti-nu-cle-on
  anti-rev-o-lu-tion-ary
  a-peri-odic
  apoth-e-o-ses
  apoth-e-o-sis
  ap-pen-di-ces
  ap-pen-dix
  ap-pen-dixes
  ar-chi-me-dean
  ar-chi-pel-ago
  ar-chi-pel-a-gos
  ar-chive
  ar-chives
  ar-chiv-ing
  ar-chiv-ist
  ar-chiv-ists
  ar-che-typ-al
  ar-che-type
  ar-che-types
  ar-che-typ-i-cal
  arc-tan-gent
  arc-tan-gents
  a-spher-ic
  a-spher-i-cal
  as-sign-a-ble
  as-sign-or
  as-sign-ors
  as-sist-ant
  as-sist-ance
  as-sist-ant-ship
  as-sist-ant-ships
  as-trol-o-ger
  as-trol-o-gers
  as-tron-o-mer
  as-tron-o-mers
  asymp-to-matic
  as-ymp-tot-ic
  asyn-chro-nous
  ath-er-o-scle-ro-sis
  at-mos-phere
  at-mos-pheres
  at-tri-bute
  at-trib-uted
  at-trib-ut-able
  au-to-ma-tion
  au-tom-a-ton
  au-tom-a-ta
  auto-num-ber-ing
  au-ton-o-mous
  auto-re-gres-sion
  auto-re-gres-sive
  auto-round-ing
  av-oir-du-pois
  back-scratcher
  back-scratch-ing
  band-lead-er
  band-lead-ers
  bank-rupt
  bank-rupts
  bank-rupt-cy
  bank-rupt-cies
  bar-onies
  base-line-skip
  ba-thym-e-try
  bathy-scaphe
  bean-ies
  be-drag-gle
  be-drag-gled
  bed-rid-den
  bed-rock
  be-dwarf
  be-dwarfs
  be-hav-iour
  be-hav-iours
  bevies
  bib-lio-graph-i-cal
  bib-li-og-ra-phy-style
  bib-units
  bi-dif-fer-en-tial
  big-gest
  big-shot
  big-shots
  bill-able
  bio-math-e-mat-ics
  bio-med-i-cal
  bio-med-i-cine
  bio-rhythms
  bio-weap-ons
  bio-weap-on-ry
  bit-map
  bit-maps
  bland-er
  bland-est
  blind-er
  blind-est
  blondes
  blue-print
  blue-prints
  bo-lom-e-ter
  bo-lom-e-ters
  book-sell-er
  book-sell-ers
  bool-ean
  bool-eans
  bor-no-log-i-cal
  bot-u-lism
  brusquer
  buf-fer
  buf-fers
  bun-gee
  bun-gees
  busier
  busi-est
  bussing
  butted
  buzz-word
  buzz-words
  cache-abil-ity
  cache-able
  ca-coph-o-ny
  ca-coph-o-nies
  call-er
  call-ers
  cam-era-men
  cart-wheel
  cart-wheels
  ca-tarrh
  ca-tarrhs
  ca-tas-tro-phe
  ca-tas-tro-phes
  cat-a-stroph-ic
  cat-a-stroph-i-cally
  ca-tas-tro-phism
  cat-e-noid
  cat-e-noids
  cau-li-flow-er
  chan-cery
  chap-ar-ral
  char-treuse
  chemo-kine
  chemo-kines
  chemo-ther-apy
  chemo-ther-a-pies
  chloro-meth-ane
  chloro-meth-anes
  cho-les-teric
  cig-a-rette
  cig-a-rettes
  cinque-foil
  co-asso-cia-tive
  coch-leas
  coch-lear
  co-designer
  co-designers
  co-gnac
  co-gnacs
  co-ker-nel
  co-ker-nels
  col-lin-ea-tion
  col-umns
  com-par-and
  com-par-ands
  com-pen-dium
  com-po-nent-wise
  comp-trol-ler
  comp-trol-lers
  com-put-able
  com-put-abil-ity
  con-form-able
  con-form-ist
  con-form-ists
  con-form-ity
  con-ge-ries
  con-gress
  con-gresses
  con-struc-ted
  con-struc-ti-ble
  con-struc-ti-bil-ity
  con-trib-ute
  con-trib-utes
  con-trib-uted
  copy-right-able
  co-re-la-tion
  co-re-la-tions
  co-re-li-gion-ist
  co-re-li-gion-ists
  co-re-op-sis
  co-re-spon-dent
  co-re-spon-dents
  co-se-cant
  co-semi-sim-ple
  co-tan-gent
  cour-ses
  co-work-er
  co-work-ers
  crank-case
  crank-shaft
  croc-o-dile
  croc-o-diles
  cross-hatch
  cross-hatched
  cross-hatch-ing
  cross-over
  cryp-to-gram
  cryp-to-grams
  cuff-link
  cuff-links
  cu-nei-form
  cus-tom-iz-a-ble
  cus-tom-ize
  cus-tom-izes
  cus-tom-ized
  cy-ber-virus
  cy-ber-viruses
  cy-ber-wea-pon
  cy-ber-wea-pons
  cy-to-kine
  cy-to-kines
  dachs-hund
  dam-sel-fly
  dam-sel-flies
  dactyl-o-gram
  dactyl-o-graph
  data-base
  data-bases
  data-path
  data-paths
  date-stamp
  date-stamps
  de-allo-cate
  de-allo-cates
  de-allo-cated
  de-allo-ca-tion
  de-allo-ca-tions
  de-clar-able
  de-fin-i-tive
  de-lec-ta-ble
  demi-semi-qua-ver
  demi-semi-qua-vers
  de-moc-ra-tism
  demos
  der-i-va-tion
  der-i-va-tions
  der-i-va-tion-al
  de-riv-a-tive
  de-riv-a-tives
  dia-lec-tic
  dia-lec-tics
  dia-lec-ti-cian
  dia-lec-ti-cians
  di-chloro-meth-ane
  dif-fract
  dif-fracts
  dif-frac-tion
  dif-frac-tions
  direr
  dire-ness
  dis-par-and
  dis-par-ands
  dis-traught-ly
  dis-trib-ut-able
  dis-trib-ute
  dis-trib-utes
  dis-trib-uted
  dis-trib-u-tive
  dou-ble-space
  dou-ble-spaced
  dou-ble-spac-ing
  dou-ble-talk
  doll-ish
  drift-age
  driv-ers
  drom-e-dary
  drom-e-daries
  drop-let
  drop-lets
  du-op-o-list
  du-op-o-lists
  du-op-o-ly
  du-op-o-lies
  dys-lexia
  dys-lec-tic
  dys-topia
  east-end-ers
  eco-sys-tem
  eco-sys-tems
  eco-nom-ics
  econ-o-mies
  econ-o-mist
  econ-o-mists
  ei-gen-class
  ei-gen-classes
  ei-gen-val-ue
  ei-gen-val-ues
  electro-mechan-i-cal
  electro-mechano-acoustic
  elec-tro-pho-re-sis
  elec-tro-pho-ret-ic
  elit-ist
  elit-ists
  en-dos-copy
  en-dos-copies
  en-tre-pre-neur
  en-tre-pre-neurs
  en-tre-pre-neur-ial
  ep-i-neph-rine
  eps-to-pdf
  equi-vari-ant
  equi-vari-ance
  er-go-nom-ic
  er-go-nom-ics
  er-go-nom-i-cally
  es-sence
  es-sences
  eth-ane
  eth-yl-am-ine
  eth-yl-ate
  eth-yl-ated
  eth-yl-ene
  ethy-nyl
  ethy-nyl-a-tion
  eu-sta-chian
  ever-si-ble
  evert
  everts
  evert-ed
  evert-ing
  ex-plan-a-tory
  ex-quis-ite
  ex-tra-or-di-nary
  face-lifts
  face-lift-ing
  fall-ing
  fermi-ons
  figu-rine
  figu-rines
  fi-nite-ly
  fla-gel-lum
  fla-gel-la
  flam-ma-bles
  fledg-ling
  flow-chart
  flow-charts
  fluoro-car-bon
  fluor-os-copies
  fluor-os-copy
  for-mi-da-ble
  for-mi-da-bly
  for-syth-ia
  forth-right
  free-loader
  free-loaders
  friend-lier
  friend-li-est
  fri-vol-ity
  fri-vol-i-ties
  friv-o-lous
  front-end
  front-ends
  ga-lac-tic
  gal-axy
  gal-ax-ies
  gaz-et-teer
  gaz-et-teers
  gas-om-e-ter
  ge-o-des-ic
  ge-o-det-ic
  ge-om-eter
  ge-om-eters
  geo-met-ric
  geo-met-rics
  ge-o-strophic
  geo-ther-mal
  ge-ot-ro-pism
  giga-nodes
  gno-mon
  gno-mons
  gran-di-ose
  grand-uncle
  grand-uncles
  griev-ance
  griev-ances
  griev-ous
  griev-ous-ly
  group-like
  hair-style
  hair-styles
  hair-styl-ist
  hair-styl-ists
  half-life
  half-lives
  half-space
  half-spaces
  half-tone
  half-tones
  half-way
  har-bin-ger
  har-bin-gers
  har-le-quin
  har-le-quins
  hatch-eries
  hei-nous
  he-lio-pause
  he-lio-trope
  hemi-demi-semi-qua-ver
  hemi-demi-semi-qua-vers
  he-mo-glo-bin
  he-mo-phil-ia
  he-mo-phil-iac
  he-mo-phil-iacs
  hemo-rhe-ol-ogy
  he-pat-ic
  he-pat-ica
  her-maph-ro-dite
  her-maph-ro-dit-ic
  he-roes
  hexa-dec-i-mal
  hip-po-po-ta-mus
  holo-deck
  holo-decks
  ho-lo-no-my
  ho-meo-mor-phic
  ho-meo-mor-phism
  ho-meo-stat-ic
  ho-meo-stat-ics
  ho-meo-sta-sis
  ho-mo-thetic
  horse-rad-ish
  hot-bed
  hot-beds
  hounds-teeth
  hounds-tooth
  hy-dro-ther-mal
  hy-per-elas-tic-ity
  hy-phen-a-tion
  hy-phen-a-tions
  hy-po-elas-tic-ity
  hy-po-thal-a-mus
  ico-nog-ra-pher
  ico-nog-ra-phers
  icon-o-graph-ic
  ico-nog-ra-phy
  ideals
  ideo-graphs
  idio-syn-crasy
  idio-syn-cra-sies
  idio-syn-cratic
  idio-syn-crat-i-cal-ly
  ig-nit-er
  ig-nit-ers
  ig-ni-tor
  ignore-spaces
  il-li-quid
  il-li-quid-ity
  im-mu-ni-za-tion
  im-mu-no-mod-u-la-to-ry
  im-ped-ance
  im-ped-ances
  in-du-bi-ta-ble
  in-fin-ite-ly
  in-fin-i-tes-i-mal
  in-fra-struc-ture
  in-fra-struc-tures
  input-enc
  in-stall-er
  in-stall-ers
  in-teg-rity
  in-ter-dis-ci-pli-nary
  in-ter-ga-lac-tic
  in-ter-view-ee
  in-ter-view-ees
  in-utile
  in-util-i-ty
  ir-ra-tio-nal
  ir-re-duc-ible
  ir-re-duc-ibly
  ir-rev-o-ca-ble
  iso-geo-met-ric
  iso-geo-met-rics
  iso-ther-mal
  isot-ropy
  iso-trop-ic
  itin-er-ary
  itin-er-ar-ies
  je-re-mi-ads
  key-note
  key-notes
  key-stroke
  key-strokes
  kilo-nodes
  kiln-ing
  lac-i-est
  lam-en-ta-ble
  land-scap-er
  land-scap-ers
  lar-ce-n
  lar-ce-ny
  lar-ce-nies
  lar-ce-nist
  leaf-hop-per
  leaf-hop-pers
  leaf-let
  leaf-lets
  let-ter-spaces
  let-ter-spaced
  let-ter-spac-ing
  leu-ko-cyte
  leu-ko-cytes
  leu-ko-triene
  leu-ko-trienes
  life-span
  life-spans
  life-style
  life-styles
  lift-off
  light-weight
  lim-ou-sines
  line-backer
  line-spacing
  li-on-ess
  li-quid-ity
  lith-o-graphed
  lith-o-graphs
  lo-bot-omy
  lo-bot-om-ize
  loges
  long-est
  look-ahead
  lo-quac-ity
  love-struck
  macro-eco-nomic
  macro-eco-nomics
  macro-econ-omy
  make-in-dex
  mal-a-prop-ism
  mal-a-prop-isms
  man-slaugh-ter
  man-u-script
  man-u-scripts
  mar-gin-al
  math-e-ma-ti-cian
  math-e-ma-ti-cians
  mattes
  med-ic-aid
  medi-ocre
  medi-oc-ri-ties
  mega-fau-na
  mega-fau-nal
  mega-lith
  mega-liths
  mega-nodes
  meta-bol-ic
  me-tab-o-lism
  me-tab-o-lisms
  me-tab-o-lite
  me-tab-o-lites
  meta-form
  meta-forms
  meta-lan-guage
  meta-lan-guages
  meta-phor
  meta-phors
  meta-phor-i-cal
  meta-phor-i-cal-ly
  meta-sta-bil-ity
  meta-stable
  meta-table
  meta-tables
  metem-psy-cho-sis
  meth-am-phet-a-mine
  meth-ane
  meth-od
  meth-yl-am-mo-nium
  meth-yl-ate
  meth-yl-ated
  meth-yl-a-tion
  meth-yl-ene
  me-trop-o-lis
  me-trop-o-lises
  met-ro-pol-i-tan
  met-ro-pol-i-tans
  micro-eco-nomic
  micro-eco-nomics
  micro-econ-omy
  micro-en-ter-prise
  micro-en-ter-prises
  mi-cro-fiche
  mi-cro-fiches
  micro-organ-ism
  micro-organ-isms
  mi-cro-struc-ture
  mid-after-noon
  mill-age
  mil-li-liter
  mimeo-graphed
  mimeo-graphs
  mim-ic-ries
  mine-sweeper
  mine-sweepers
  min-is
  mini-sym-po-sium
  mini-sym-po-sia
  mi-nut-er
  mi-nut-est
  mis-chie-vous-ly
  mi-sers
  mi-sog-a-my
  mne-mon-ic
  mne-mon-ics
  mod-el-ling
  mo-lec-u-lar
  mol-e-cule
  mol-e-cules
  mon-archs
  money-len-der
  money-len-ders
  mono-chrome
  mono-en-er-getic
  mon-oid
  mon-oph-thong
  mon-oph-thongs
  mono-pole
  mono-poles
  mo-nop-oly
  mono-space
  mono-spaced
  mono-spacing
  mono-spline
  mono-splines
  mono-strofic
  mo-not-o-nies
  mo-not-o-nous
  mo-ron-ism
  mos-qui-to
  mos-qui-tos
  mos-qui-toes
  mud-room
  mud-rooms
  mul-ti-fac-eted
  mul-ti-plic-able
  mul-ti-plic-ably
  multi-user
  name-space
  name-spaces
  neo-fields
  neo-nazi
  neo-nazis
  neph-ews
  neph-rite
  neph-ritic
  new-est
  news-let-ter
  news-let-ters
  nil-po-tent
  nitro-meth-ane
  node-list
  node-lists
  no-name
  non-ar-ith-met-ic
  non-emer-gency
  non-equi-vari-ance
  none-the-less
  non-euclid-ean
  non-iso-mor-phic
  non-pseudo-com-pact
  non-smooth
  non-uni-form
  non-uni-form-ly
  non-zero
  nor-ep-i-neph-rine
  not-with-stand-ing
  nu-cleo-tide
  nu-cleo-tides
  nut-crack-er
  nut-crack-ers
  oer-steds
  off-line
  off-load
  off-loads
  off-loaded
  oli-gop-o-list
  oli-gop-o-lists
  oli-gop-oly
  oli-gop-ol-ies
  om-ni-pres-ent
  om-ni-pres-ence
  ono-mat-o-poe-ia
  ono-mat-o-po-et-ic
  op-er-and
  op-er-ands
  orang-utan
  orang-utans
  or-tho-don-tist
  or-tho-don-tists
  or-tho-ker-a-tol-ogy
  ortho-nitro-toluene
  over-view
  over-views
  ox-id-ic
  pad-ding
  page-rank
  pain-less-ly
  pal-ette
  pal-ettes
  pa-rab-ola
  par-a-bol-ic
  pa-rab-o-loid
  par-a-digm
  par-a-digms
  para-chute
  para-chutes
  para-di-methyl-benzene
  para-fluoro-toluene
  para-graph-er
  para-le-gal
  par-al-lel-ism
  para-mag-net-ism
  para-medic
  para-methyl-anisole
  pa-ram-e-tri-za-tion
  pa-ram-e-trize
  para-mil-i-tary
  para-mount
  path-o-gen-ic
  peev-ish
  peev-ish-ness
  pen-al-ty
  pen-al-ties
  pen-ta-gon
  pen-ta-gons
  pe-tro-le-um
  phe-nol-phthalein
  phe-nom-e-non
  phenyl-ala-nine
  phi-lat-e-list
  phi-lat-e-lists
  pho-neme
  pho-nemes
  pho-ne-mic
  phos-phor-ic
  pho-to-graphs
  pho-to-off-set
  phtha-lam-ic
  phthal-ate
  phthi-sis
  pic-a-dor
  pic-a-dors
  pipe-line
  pipe-lines
  pipe-lin-ing
  pi-ra-nhas
  placa-ble
  plant-hop-per
  plant-hop-pers
  pla-teau
  pla-teaus
  pleas-ance
  plug-in
  plug-ins
  pol-ter-geist
  poly-an-dr
  poly-an-dry
  poly-an-drous
  poly-dac-tyl
  poly-dac-tyl-lic
  poly-ene
  poly-eth-yl-ene
  po-lyg-a-mist
  po-lyg-a-mists
  polyg-on-i-za-tion
  po-lyg-y-n
  po-lyg-y-ny
  po-lyg-y-nous
  pol-yp
  pol-yps
  po-lyph-o-n
  po-lyph-o-ny
  po-lyph-o-nous
  poly-phon-ic
  poly-styrene
  pome-gran-ate
  poro-elas-tic
  por-ous
  por-ta-ble
  post-am-ble
  post-am-bles
  post-hu-mous
  post-script
  post-scripts
  pos-tur-al
  pre-am-ble
  pre-am-bles
  pre-dict-able
  pre-fers
  pre-loaded
  pre-par-ing
  pre-print
  pre-prints
  pre-proces-sor
  pre-proces-sors
  pres-ent-ly
  pre-split-ting
  pre-wrap
  pre-wrapped
  priest-esses
  pret-ty-prin-ter
  pret-ty-prin-ting
  pro-ce-dur-al
  process
  pro-cur-ance
  prog-e-nies
  prog-e-ny
  pro-gram-mable
  pro-kary-ote
  pro-kary-otes
  pro-kary-ot-ic
  prom-i-nent
  pro-mis-cu-ous
  prom-is-sory
  prom-ise
  prom-ises
  pro-pel-ler
  pro-pel-lers
  pro-pel-ling
  pro-hib-i-tive
  pro-hib-i-tive-ly
  pro-sciut-to
  pros-ta-glan-din
  pros-ta-glan-dins
  pro-style
  pro-styles
  pro-test-er
  pro-test-ers
  pro-tes-tor
  pro-tes-tors
  pro-to-lan-guage
  pro-to-typ-al
  prov-ince
  prov-inces
  pro-vin-cial
  pro-virus
  pro-viruses
  prow-ess
  pseu-do-dif-fer-en-tial
  pseu-do-fi-nite
  pseu-do-fi-nite-ly
  pseu-do-forces
  pseu-dog-ra-pher
  pseu-do-group
  pseu-do-groups
  pseu-do-nym
  pseu-do-nyms
  pseu-do-word
  pseu-do-words
  psy-che-del-ic
  psychs
  pu-bes-cence
  pur-ges
  quad-ding
  qua-drat-ic
  qua-drat-ics
  quad-ra-ture
  quad-ri-lat-er-al
  quad-ri-lat-er-als
  quad-ri-pleg-ic
  quad-ru-ped
  quad-ru-peds
  quad-ru-pole
  quad-ru-poles
  quaint-er
  quaint-est
  qua-si-equiv-a-lence
  qua-si-equiv-a-lences
  qua-si-equiv-a-lent
  qua-si-hy-po-nor-mal
  qua-si-rad-i-cal
  qua-si-resid-ual
  qua-si-smooth
  qua-si-sta-tion-ary
  qua-si-topos
  qua-si-tri-an-gu-lar
  qua-si-triv-ial
  quin-tes-sence
  quin-tes-sences
  quin-tes-sen-tial
  rab-bit-ry
  ra-di-og-ra-phy
  raff-ish
  raff-ish-ly
  ram-shackle
  rav-en-ous
  re-allo-cate
  re-allo-cates
  re-allo-cated
  re-arrange
  re-arranges
  re-arranged
  re-arrange-ment
  re-arrange-ments
  rec-i-proc-i-ties
  rec-i-proc-i-ty
  rec-tan-gle
  rec-tan-gles
  rec-tan-gu-lar
  re-di-rect
  re-di-rect-ion
  re-duc-ible
  re-echo
  re-edu-cate
  ref-u-gee
  ref-u-gees
  re-imple-ment
  re-imple-ments
  re-imple-mented
  re-imple-men-ta-tion
  ren-ais-sance
  re-phrase
  re-phrases
  re-phrased
  re-po-si-tion
  re-po-si-tions
  re-print
  re-prints
  re-print-ed
  re-stor-able
  retro-fit
  retro-fit-ted
  re-us-able
  re-use
  re-wire
  re-wrap
  re-wrapped
  re-write
  rhi-noc-er-os
  right-eous
  right-eous-ness
  ring-leader
  ring-leaders
  ro-bot
  ro-bots
  ro-botic
  ro-bot-ics
  roof-top
  roof-tops
  round-table
  round-tables
  sales-clerk
  sales-clerks
  sales-woman
  sales-women
  sa-lient
  sal-mo-nel-la
  sal-ta-tion
  sar-sa-par-il-la
  sat-el-lite
  sat-el-lites
  sauer-kraut
  scat-o-log-i-cal
  scene-shift-er
  scene-shift-ing
  sched-ul-ing
  schiz-o-phrenic
  schnau-zer
  school-child
  school-child-ren
  school-teacher
  school-teach-ers
  scru-ti-ny
  scyth-ing
  sell-er
  sell-ers
  sec-re-tar-iat
  sec-re-tar-iats
  sem-a-phore
  sem-a-phores
  se-mes-ter
  semi-def-i-nite
  semi-di-rect
  semi-ho-mo-thet-ic
  semi-ring
  semi-rings
  semi-sim-ple
  semi-skilled
  sem-itic
  ser-geant
  ser-geants
  sero-epi-de-mi-o-log-i-cal
  ser-vo-me-chan-i-cal
  ser-vo-mech-a-nism
  ser-vo-mech-a-nisms
  ses-qui-pe-da-lian
  set-up
  set-ups
  se-vere-ly
  shap-able
  shape-able
  shoe-string
  shoe-strings
  shop-lift-er
  shop-lift-ing
  show-hy-phens
  side-step
  side-steps
  side-swipe
  sign-age
  single-space
  single-spaced
  single-spacing
  sky-scraper
  sky-scrapers
  sln-uni-code
  smoke-stack
  smoke-stacks
  snor-kel-ing
  so-le-noid
  so-le-noids
  solute
  solutes
  sov-er-eign
  sov-er-eigns
  spa-ces
  spe-cious
  spell-er
  spell-ers
  spell-ing
  spe-lunk-er
  spend-thrift
  spher-oid
  spher-oids
  spher-oid-al
  sphin-ges
  spic-i-ly
  spin-or
  spin-ors
  spokes-man
  spokes-per-son
  spokes-per-sons
  spokes-woman
  spokes-women
  sports-cast
  sports-cast-er
  spor-tive-ly
  sports-wear
  sports-writer
  sports-writers
  spright-lier
  squea-mish
  stand-alone
  star-tling
  star-tling-ly
  sta-tis-tics
  stealth-ily
  steeple-chase
  stereo-graph-ic
  sto-chas-tic
  strange-ness
  strap-hanger
  strat-a-gem
  strat-a-gems
  stretch-i-er
  strip-tease
  strong-est
  strong-hold
  stu-pid-er
  stu-pid-est
  sub-dif-fer-en-tial
  sub-ex-pres-sion
  sub-ex-pres-sions
  sub-node
  sub-nodes
  sub-scrib-er
  sub-scrib-ers
  sub-tables
  sum-ma-ble
  super-deri-va-tion
  super-deri-va-tions
  super-ego
  super-egos
  su-prem-a-cist
  su-prem-a-cists
  sur-gery
  sur-ge-ries
  sur-ges
  sur-veil-lance
  swim-ming-ly
  symp-to-matic
  syn-chro-mesh
  syn-chro-nous
  syn-chro-tron
  taff-rail
  take-over
  take-overs
  talk-a-tive
  ta-pes-try
  ta-pes-tries
  tar-pau-lin
  tar-pau-lins
  te-leg-ra-pher
  te-leg-ra-phers
  tele-ki-net-ic
  tele-ki-net-ics
  tele-ro-bot-ics
  tell-er
  tell-ers
  tem-po-rar-ily
  ten-ure
  test-bed
  tera-nodes
  tetra-butyl-ammo-nium
  text-height
  text-length
  text-width
  thal-a-mus
  ther-mo-elas-tic
  time-stamp
  time-stamps
  tool-kit
  tool-kits
  topo-graph-i-cal
  topo-iso-mer-ase
  topo-iso-mer-ases
  toques
  trai-tor-ous
  trans-ceiver
  trans-ceivers
  trans-par-en-cy
  trans-par-en-cies
  trans-gress
  trans-ver-sal
  trans-ver-sals
  trans-ves-tite
  trans-ves-tites
  tra-vers-a-ble
  tra-ver-sal
  tra-ver-sals
  tri-ethyl-amine
  treach-eries
  tribes-man
  trip-let
  trip-lets
  tri-plex
  tri-plex-es
  trou-ba-dour
  tur-key
  tur-keys
  turn-around
  turn-arounds
  typ-al
  un-at-tached
  un-err-ing-ly
  un-friend-ly
  un-friend-li-er
  un-in-stan-ti-at-ed
  vaguer
  vaude-ville
  vic-ars
  vil-lain-ess
  vis-ual
  vis-ual-ly
  vi-vip-a-rous
  voice-print
  vspace
  wad-ding
  wall-flower
  wall-flow-ers
  warm-er
  warm-est
  waste-water
  wave-guide
  wave-guides
  wave-let
  wave-lets
  weap-ons
  weap-on-ry
  web-like
  web-log
  web-logs
  week-night
  week-nights
  weight-lift-er
  weight-lift-ing
  wheel-chair
  wheel-chairs
  which-ever
  white-sided
  white-space
  white-spaces
  wide-spread
  wing-span
  wing-spans
  wing-spread
  witch-craft
  word-spac-ing
  work-around
  work-arounds
  work-horse
  work-horses
  wrap-around
  wrap-arounds
  wretch-ed
  wretch-ed-ly
  yes-ter-year
  Alex-an-der
  Alex-an-drine
  al-ge-brai-sche
  Al-gon-quian
  Al-gon-quin
  Al-le-ghe-ny
  Apol-lo-dorus
  Ar-kan-sas
  ATP-ase
  ATP-ases
  Auf-lage
  Aus-tral-asian
  auto-ma-ti-sier-ter
  Beb-chuk
  Be-die-nung
  Bembo
  bi-blio-gra-phi-sche
  Bos-ton
  Brown-ian
  Bruns-wick
  Bu-da-pest
  Burck-hardt
  Cara-theo-dory
  Car-ib-bean
  Charles-ton
  Char-lottes-ville
  Ches-ter
  Chiang
  Chich-es-ter
  Cohen
  Co-lum-bia
  Czecho-slo-va-kia
  Del-a-ware
  Dijk-stra
  Dor-ches-ter
  Dorf-leit-ner
  Drechs-ler
  Duane
  dy-na-mi-sche
  Eijk-hout
  Engle
  Engel
  Eng-lish
  Euler-ian
  Evan-ston
  Feb-ru-ary
  Fest-schrift
  Flor-i-da
  Flor-i-d-ian
  For-schungs-in-sti-tut
  Free-BSD
  funk-tsional
  Gauss-ian
  Ge-sell-schaft
  Ghost-script
  Ghost-View
  Gott-fried
  Gott-lieb
  Grass-mann-ian
  Greifs-wald
  Grothen-dieck
  Grund-leh-ren
  Ha-da-mard
  Hai-fa
  Hamil-ton-ian
  Hel-sinki
  Her-mit-ian
  Hibbs
  Hoef-ler
  Hoek-water
  Hok-kai-do
  Huber
  Image-Magick
  Jac-kow-ski
  Jan-u-ary
  Ja-pa-nese
  Java-Script
  Jung-ian
  Kad-om-tsev
  Kan-sas
  Karls-ruhe
  Keynes-ian
  Kor-te-weg
  Krishna
  Krish-na-ism
  Krish-nan
  Kron-ecker
  Lan-cas-ter
  Le-gendre
  Leices-ter
  Lip-schitz
  Lip-schitz-ian
  Loj-ban
  Lou-i-si-ana
  Lucas
  MacBeth
  Mac-OS
  Ma-gel-lan
  Ma-la-ya-lam
  Man-ches-ter
  Mar-kov-ian
  Markt-ober-dorf
  Mass-a-chu-setts
  Max-well
  Meth-od-ist
  Meth-od-ism
  Mi-cro-soft
  Min-kow-ski
  Min-ne-ap-o-lis
  Min-ne-sota
  Mont-real
  Mos-cow
  Nach-rich-ten
  Nash-ville
  Net-BSD
  Net-scape
  Nietz-sche
  Nij-me-gen
  Noe-ther-ian
  Noord-wijker-hout
  Noto-wi-digdo
  No-vem-ber
  Obst-feld
  Open-BSD
  Open-Office
  Oreo-pou-los
  Pala-tino
  Pa-ler-mo
  Pe-trov-ski
  Pfaff-ian
  Phil-a-del-phia
  phi-lo-so-phi-sche
  Poin-care
  Po-ten-tial-glei-chung
  Po-to-mac
  Pres-by-terian
  Pres-by-terians
  Pyong-yang
  Py-thag-o-ras
  Py-thag-o-re-an
  Ra-dha-krish-nan
  raths-kel-ler
  Ravi-kumar
  Reich-lin
  Rie-mann-ian
  Ryd-berg
  Schim-mel-pfen-nig
  schot-ti-sche
  Schro-din-ger
  Schwa-ba-cher
  Schwarz-schild
  Schweid-nitz
  Schwert
  Sep-tem-ber
  Shore-ditch
  Skoup
  Stokes-sche
  Stutt-gart
  Sus-que-han-na
  Tau-ber-ian
  tech-ni-sche
  Ten-nes-see
  Thiruv-ananda-puram
  Tol-ches-ter
  To-ma-szew-ski
  Toyo-ta
  ty-po-graphique
  Ukrain-ian
  ver-all-ge-mei-nerte
  Ver-ei-ni-gung
  Ver-tei-lun-gen
  Vid-ias-sov
  Vieth
  viiith
  viith
  Wahr-schein-lich-keits-theo-rie
  Wein-stein
  Werk-zeuge
  Wer-ner
  Wer-ther-ian
  Will-iam
  Will-iams
  Win-ches-ter
  Wirt-schaft
  wis-sen-schaft-lich
  Wolff-ian
  xviiith
  xviith
  xxiiird
  xxiind
  Ying-yong Shu-xue Ji-suan
  Zea-land
  Zeit-schrift
}

% EOF

==> section/notes.tex <==
\section{Notes}

\subsection{Experiment design}
\subsubsection{Baselines}
1. For range query in high dimensional data: R\*-tree, Inverted index on the CPU, GPUScan and CPUScan

2. For match query of sequence: inverted index on the CPU, GPUScan and CPUScan

3. For LSH on Euclidean space

4. For LSH on kernel space and minHash



\subsubsection{Data sets}


1. Tweets,

2. High dimensional data set (SIFT?)

2. OCR and FaceDetection (using LSH transform, check the C2LSH and SRS)

3. Adult Data Set (48K, we may increase the size of it)

4. MinHash data (NSF Research Award Abstracts 1990-2003 Data Set or WikiPedia)



\subsection{Experiment}
\subsubsection{Topk-search on adaptive Threshold}
1. query number V.S. running time on Tweets, SIFT, OCR and FD, and document data?, Adult Data Set  for range search. http://archive.ics.uci.edu/ml/datasets/Adult
2. query number V.S. unit running time on Tweets

\subsubsection{varying data size}

\subsubsection{flexible range constraint search}
Similar with Topk-search on adaptive Threshold, SIFT and OCR may be on original space

\subsubsection{Effectiveness of load balance}

\subsubsection{Comparison with different Genie method}
Genie-full, Genie-Bitmap, Genie-hash table, Genie-naive index (run by wenhao)

\subsubsection{time profiling on different stage of top-k and range search}

\subsubsection{prediction performance on OCR, FD and match count}

\subsection{Requirement for tweets data}
1. Topk-search on adaptive Threshold, query range: {32,64, 128, 256, 512, 1024, 2048, 4096 ...} (try the maximum number of queries)


2. varying data size: 500K, 1M, 2M, 4M, 7M with fixed query = 1024

3.  time profiling: 7M with fixed query 1024, stage:

4. topk-search with query range on Genie-full, Genie-Bitmap, Genie-hash table, Genie-naive index



\subsection{Data for match count}
candidate data sets:
1. Adult Data Set 48K, http://archive.ics.uci.edu/ml/datasets/Adult

2. Additional competitor, SQLite

3. to range query with different methods

3. varying data size

\subsection{Requirement for SIFT data}
1. How determine the number of hash tables for SIFT data?

2. How to determine the initial bucket width

3.  time profiling: 7M with fixed query 1024, stage:

4. Topk-search on adaptive Threshold, query range: {32,64, 128, 256, 512, 1024, 2048, 4096 ...} (try the maximum number of queries)

5. Add one special experiment: SIFT range search on original space, v.s. R-tree

\subsection{Requirement for OCR and FD data set}
1. for step 1-4, similar with the SIFT data

2. add one experiment to see the prediction performance based on 1-NN kernel distance, V.S. the 1-NN on R-tree with original space, and 1-NN with scan by kernel space


\subsection{Requirement for MinHash Dataset}
Similar with the OCR and FD data set

%2. microblogPCU Data Set
%http://archive.ics.uci.edu/ml/datasets/microblogPCU


\section{Some notes about papers}
\subsection{notes about the hash table}
The implementation of the lock-free hash table on GPU requires a bulk execution model [7] to group multiple hash
table operations within a batch and to execute the batch on GPU as a single task. The operations within the batch are
executed concurrently on the GPU.  --\ref{moazeni2012lock}





\section{Note for related works}

\subsection{importance of GPU}

 In high performance computing area,  GPUs as accelerators have already been widely deployed to process performance-critical tasks

 , in the database area, we can hardly find any major
data warehousing system (e.g., Teradata, DB2, Oracle,
SQL Server) or MapReduce-based data analytical system
(e.g., Hive, Pig, Tenzing) that has truely adopted GPUs for
productions, despite the existence of many research papers
optimizing various database operations on GPUs which have
already shown the significant performance benefits when utilizing
GPUs.


2. computing device:
neural networks, matrix solvers

3.The massively parallel GPU architectures and their highperformance
floating point arithmetic operations have been shown
well-suited for large scale scientific data analysis applications. \cite{kim2013parallel}


5. Where is the Data? Why You Cannot Debate CPU vs. GPU Performance Without the Answer \cite{gregg2011data}

. Therefore, it is necessary to either include memory transfer overhead when reporting GPU performance, or
to explain why this is not relevant for the application in question



\subsection{writing note}
1. migrate to the GPU-based data base.  (like the spark from disk to memory)

\subsection{paper note}



 \subsubsection{query optimization on the GPU}

4.  Accelerating SQL Database Operations on a GPU with CUDA \cite{bakkum2010accelerating}

accelerating database operations by offloading queries to a GPU

 11. A fast similarity join algorithm using graphics processing units \cite{lieberman2008fast}
 12. High-throughput transaction executions on graphics processors \cite{he2011high}
 uses bulk execution model to group multiple transactions into a bulk and execute the bulk as a single task on GPU.

 13. Relational joins on graphics processors \cite{he2008relational}
 14 Relational query coprocessing on graphics processors \cite{he2009relational}
 15. Fast computation of database operations using graphics processors \cite{govindaraju2004fast}


3. The yin and yang of processing data warehousing queries on GPU devices \cite{yuan2013yin}
http://web.cse.ohio-state.edu/hpcs/WWW/HTML/publications/abs13-2.html

two basic factors of GPU query processing
he Yin represents PCIe data transfer,
which transfers data between host memory and GPU device
memory. The Yang represents kernel execution, which
executes the query on the data stored in the GPU device
memory


20. MapD: \cite{mapd2015}
query operations, with the tweets visualization
MapD is not just a parallel database that runs on GPUs, it is also a visualization system that runs on those same GPUs, and this is one of the secrets of the program


\subsubsection{inverted index}
8. Using Graphics Processors for High Performance IR Query Processing \cite{ding2009using}
We present a new GPU-based system architecture for IR query processing

 inverted index compression techniques for GPU

 intersecting inverted lists on
GPUs, based on techniques from the literature on parallel
merging

9. Efficient Parallel Lists Intersection and Index Compression Algorithms using Graphics Processing Units \cite{ao2011efficient}
(similar with 8)
We investigate new approaches to improve two important
operations of search engines – lists intersection and index
compression

\subsubsection{tree structure on GPU}
 16. Parallel implementation of R-trees on the GPU \cite{luo2012parallel}
 17. Parallel multi-dimensional range query processing with R-trees on GPU \cite{kim2013parallel}

 18 Implementing database operations using SIMD instructions \cite{zhou2002implementing}
 described how SIMD (Single Instruction Multiple Data) techniques can be employed
to efficiently search B+-tree

4.  Accelerating SQL Database Operations on a GPU with CUDA \cite{bakkum2010accelerating}
Fix et al. proposed braided
parallelism for traversing B+-trees, wherein a single B+-Tree
exists in GPU memory and multiple independent queries are
concurrently executed within each SMP [9]

10. Glift: Generic, efficient, random-access GPU data structures \cite{lefohn2006glift}
 The structures, a stack, quadtree, and octree, are explained using simple Glift concepts and implemented using reusable Glift components. We also describe two applications of these structures not previously demonstrated on GPUs: adaptive shadow maps and octree three-dimensional paint.

FAST: fast architecture sensitive tree search on modern CPUs and GPUs\cite{kim2010fast}
a index traversal  for binary tree

\subsubsection{kNN}
 6. LSH on the GPU \cite{pan2011fast,pan2012bi}

 survey of lsh \cite{wang2014hashing}
paper: Hashing for Similarity Search: A Survey\cite{wang2014hashing}



 \subsubsection{hash table}

 Graphic applications do not need a persistent hash table;
instead, they need hash tables to be quickly constructed,
such as [5].

Coherent parallel hashing\cite{garcia2011coherent}
Real-time parallel hashing on the GPU \cite{alcantara2009real}




\subsubsection{key-value store}
1. Mega-KV: A Case for GPUs to Maximize the Throughput of In-Memory Key-Value Stores \cite{zhang2015mega}

: using GPU as the accelerator for the in-memory key-value store
http://web.cse.ohio-state.edu/hpcs/WWW/HTML/publications/papers/TR-15-1.pdf
similar paper:
2. Characterizing and evaluating a key-value store application on heterogeneous CPU-GPU systems \cite{hetherington2012characterizing}
Paper \cite{zhang2015mega} and \cite{hetherington2012characterizing} are heterogeneous CPU-GPU systems for key-value store.


7. Mars: a MapReduce framework on graphics processors \cite{he2008mars}
Since MapReduce has been
successful in easing the development of web data analysis tasks,
we propose a GPU-based MapReduce for these applications. With
the GPU-based framework, the developer writes their code using
the simple and familiar MapReduce interfaces.




\subsection{Todo list}
1. re-draw figures on excel

2. why [\textbf{TODO} why the running time of GPU-LSH is stable] in Figure \ref{fig:exp:total_time_vs_num_data}

3. change GEN-naive to GEN-noCH

4. draw Figure \ref{fig:exp:genie_vs_genie_noch}

5. Fill the result of Table \ref{tab:pred_ocr}

6. %no\_LB_match to noLB\_match

7. change string search to "short document search"

8. GPU-Idx as GPU-idx


9. re-running the experiment for precision and recall of GPU-LSH


\subsection{note for introduction}
\subsubsection{short note}
If you have time, reorganize the introduction to talke about motivation
for our work

Why generic?
Big data need to handle variety of data types through
LSH,
Shotgun and Assembly. for sequence, trees and graph
Relational data
Can be generalize by match count model

Why multi-queries?
Multi-queries
Why? SIFT features on images, Cutting an images into
pieces, sequences into qgrams, data mining


Why GPU?
Growth in GPU power, memory and speed.
Natural parallelism of inverted index processing

Then talk about
Challenges and contribution


\subsubsection{orgnization}

Shotgun and Assembly \cite{aparicio2002whole,she2004shotgun}

